Exponential Tethers for Accelerated Space Elevator Deployment

An exponential space elevator is a space elevator with a tether cross-section that varies exponentially with altitude. With such an elevator it is possible to reel in tether material at one end of the elevator while reeling out at the other end, without changing the overall taper profile. I show how to use this property to build up or clone a space elevator much more efficiently than with standard climber-based methods.

==> Makefile <==
# Add a list of home-made EPS figures here.
EPSFIGURES=

.SUFFIXES: .fig .eps .ps .dvi .bbl .bib .tex .pdf .gnuplot

FIGURES=${wildcard *.fig}
PLOTS=${wildcard *.gnuplot}
EPSFIGFILES=${FIGURES:.fig=.eps}
EPSPLOTFILES=${PLOTS:.gnuplot=.eps}
TEXFILES=*.tex

CFLAGS=-O2 -Wall
LDLIBS=-lm

PROGRAMS = maxtaper climber pullup splice splice2

all: $(PROGRAMS) ps pdf

force: rmdone all

dvi: paper.dvi

xdvi: paper.dvi
	xdvi paper.dvi

gv: paper.ps
	gv paper.ps

ps: paper.ps 

pdf: paper.pdf

rmdone:
	rm -f done.flag

done.flag:
	touch done.flag

printerrors:
	@echo "*****************************"; \
	echo Overview of typeset warnings: ; \
        echo "****************************"; \
	grep "Underfull" paper.log; \
	grep "Overfull" paper.log; \
	echo ; \
        echo "***************************"; \
	echo Overview of latex warnings: ; \
        echo "***************************"; \
	grep "LaTeX Warning" paper.log; \
        echo "***************************"; \
	echo ; \
        echo "***************************"; \
	echo Overview of bibtex warnings: ; \
        echo "***************************"; \
        grep ^Warning-- paper.blg; \
	echo "***************************"; \
	echo ; \
        echo "*************************"; \
	echo Overview of latex errors: ; \
        echo "*************************"; \
	grep "^!" paper.log; \
        echo "*************************"; \
	echo

paper.bbl: paper.bib $(TEXFILES) Makefile done.flag
	latex -interaction=batchmode paper.tex || true
	rm -f $*.dvi
	bibtex -terse $*

paper.dvi: $(TEXFILES) $(EPSPLOTFILES) $(EPSFIGFILES) $(EPSFIGURES) paper.bbl Makefile done.flag
	@echo Running latex once.; \
	while ( latex -interaction=nonstopmode paper.tex; grep Rerun paper.log ) ; do \
          echo; \
          echo "*********************************"; \
          echo "*********************************"; \
          echo Reruning to complete compilation.; \
          echo "*********************************"; \
          echo "*********************************"; \
	done; \
        echo "***************************"; \
	echo DVI file generated.; \
        echo "***************************"; \
	echo ; \
	make printerrors 
			
.dvi.pdf: Makefile
	dvips -q -t letter -P cmz -f $< | ps2pdf - $*.pdf

.fig.eps: Makefile
	fig2dev -L pstex $< $*.eps

.gnuplot.eps: Makefile
	gnuplot < $<

.dvi.ps: Makefile
	dvips -q -t letter $< -o $*.ps

.eps.pdf: Makefile
	epstopdf $<

clean:
	rm -f *.lof *.lot *.pfg *~ *.aux *.dvi *.blg *.log *.bbl $(EPSFIGFILES) *.bak paper.ps paper.pdf *.toc *.swp done.flag $(EPSPLOTFILES) *.tdat $(PROGRAMS) *.o



